Simultaneous likelihood-based bootstrap confidence sets for a large number of models

The paper studies a problem of constructing simultaneous likelihood-based confidence sets. We consider a simultaneous multiplier bootstrap procedure for estimating the quantiles of the joint distribution of the likelihood ratio statistics, and for adjusting the confidence level for multiplicity. Theoretical results state the bootstrap validity in the following setting: the sample size \(n\) is fixed, the maximal parameter dimension \(p_{\textrm{max}}\) and the number of considered parametric models \(K\) are s.t. \((\log K)^{12}p_{\max}^{3}/n\) is small. We also consider the situation when the parametric models are misspecified. If the models' misspecification is significant, then the bootstrap critical values exceed the true ones and the simultaneous bootstrap confidence set becomes conservative. Numerical experiments for local constant and local quadratic regressions illustrate the theoretical results.

==> umb_examp_locconst.tex <==
%!TEX root = simult_bootst_root.tex
%\newpage

Here we consider simultaneous confidence sets based on the local constant estimate, also known as Nadaraya-Watson estimate \cite{Nadaraya1964estimating,Watson1964smooth}.
Let \(Y_{1},\dots,Y_{n}\) be independent random scalar observations and \(X_{1},\dots,X_{n}\) some deterministic design points.
 Consider the following quadratic likelihood function reweighted with the kernel functions \(K(\cdot)\):
\begin{EQA}[c]
L(\thetav,x,h)\eqdef -\frac{1}{2}\sum\nolimits_{i=1}^{n} (Y_{i}-\thetav)^{2}w_{i}(x,h),\\
w_{i}(x,h)\eqdef K(\{x-X_{i}\}/h),\\
K(x)\in[0,1],\ \int_{\R}K(x)dx =1,\ K(x)=K(-x).
\end{EQA}
Here \(h>0\) denotes bandwidth, the local smoothing parameter. The target point and the local MLE read as:
\begin{EQA}[c]
\thetavs(x,h)\eqdef  \frac{ \sum\nolimits_{i=1}^{n}w_{i}(x,h)\E Y_{i} }{\sum\nolimits_{i=1}^{n}w_{i}(x,h)},~~~~
\thetavt(x,h)\eqdef \frac{ \sum\nolimits_{i=1}^{n}w_{i}(x,h) Y_{i} }{\sum\nolimits_{i=1}^{n}w_{i}(x,h)}.
\end{EQA}
Let us fix a bandwidth \(h\) and consider the range of points  \(x_{1},\dots,x_{\numK}\). They yield \(\numK\) local constant models with the target parameters \(\thetavs_{k}\eqdef\thetavs(x_{k},h)\) and the likelihood functions \(L_{k}(\thetav)\eqdef L(\thetav,x_{k},h)\) for \(k=1,\dots,\numK\). \begin{comment}
The confidence intervals for each model are defined as
\begin{EQA}
\CS_{k}(\zz,h)&\eqdef&\left\{\thetav\in\Theta: L(\thetavt(x_{k},h),x_{k},h)-L(\thetav,x_{k},h)\leq \zz^{2}/2\right\}.
\end{EQA}
\end{comment}

The bootstrap local likelihood function is defined similarly to the global one \eqref{def:Lbk}, by reweighting \(L(\thetav,x,h)\) with the bootstrap multipliers \(u_{1},\dots,u_{n}\):
\begin{EQA}[c]
\Lb_{k}(\thetav)\eqdef
\Lb(\thetav,x_{k},h)\eqdef -\frac{1}{2}\sum\nolimits_{i=1}^{n} (Y_{i}-\thetav)^{2}w_{i}(x_{k},h)u_{i},\\
%\end{EQA}
%and
%\begin{EQA}[c]
\thetavbt_{k}\eqdef
\thetavbt(x_{k},h)\eqdef
\frac{ \sum\nolimits_{i=1}^{n}w_{i}(x_{k},h)u_{i} Y_{i} }{\sum\nolimits_{i=1}^{n}w_{i}(x_{k},h)u_{i}}.
%\sum\limits_{i=1}^{n} \frac{ Y_{i} }{\sum\nolimits_{i=1}^{n}w_{i}(x_{k},h)u_{i}}w_{i}(x_{k},h)u_{i}.
\end{EQA}
In the numerical experiments we constructed two \(90\%\) simultaneous confidence bands: using Monte Carlo (MC) samples and bootstrap procedure with Gaussian weights (\(u_{i}\sim \mathcal{N}(1,1)\)), in each case we used \(10^{4}\) \(\{Y_{i}\}\) and \(10^{4}\) \(\{u_{i}\}\) independent samples. The sample size \(n=400\). \(K(x)\) is Epanechnikov's kernel function. The independent random observations \(Y_{i}\) are generated as follows:
\begin{EQA}[c]
\label{def:numer_Y}
Y_{i}= f(X_{i})+ \mathcal{N}(0,1),\quad
X_{i} \text{ are equidistant on } [0,1],\\
\label{def:numer_f}
f(x)=
\begin{cases}
5,& x\in [0,0.25]\cup[0.65,1];\\
5+3.8\{1-100(x-0.35)^2\},& x\in [0.25,0.45];\\
5-3.8\{1-100(x-0.55)^2\},& x\in [0.45,0.65].
\end{cases}
\end{EQA}
The number of local models \(\numK=71\), the points \(x_{1},\dots,x_{71}\) are equidistant on \([0,1]\). For the bandwidth we considered two cases: \(h=0.12\) and \(h=0.3\).

\subsection{Effect of the modeling bias on a width of a bootstrap confidence band}
The function \(f(x)\) defined in \eqref{def:numer_f} should yield a considerable modeling bias for the mean constant estimator.
Figure \ref{fig:localMLE} demonstrates that the bootstrap confidence band becomes conservative (i.e. wider than the MC confidence band) when the local constant   model is misspecified. The top graphs on Figure \ref{fig:localMLE} show the \(90\%\) confidence bands, the middle graphs show their width, and the bottom graphs show the modelling bias value for \(K=71\) local constant models (see formula \eqref{eq:numer_smb} below). For \(x\in [0.25,0.65]\) the width of the bootstrap confidence sets is considerably increased by the modeling bias. The expression for the modeling bias term for the \(k\)-th model (see also\ref{itm:SmBHk} condition) reads as:
\begin{align}
\label{eq:numer_smb}
\begin{split}
\left\|
D^{-1}_{k}B_{k}^{2}
D^{-1}_{k}
\right\|&=
\frac{\sum\nolimits_{i=1}^{n}\left\{\E Y_{i}-\thetavs(x_{k})\right\}^{2}w_{i}^{2}(x_{k},h) }
{\sum\nolimits_{i=1}^{n}\E \left\{Y_{i}-\thetavs(x_{k})\right\}^{2}w_{i}^{2}(x_{k},h) }
\\&=
1-\left(1+\frac{\sum\nolimits_{i=1}^{n}w_{i}^{2}(x_{k},h)\left\{f(X_{i})-\thetavs(x_{k})\right\}^{2}}{\sum\nolimits_{i=1}^{n}w_{i}^{2}(x_{k},h)}
\right)^{-1}.
\end{split}
\end{align}
Therefore, if \(\max_{1\leq k \leq \numK}\left\{f(X_{i})-\thetavs(x_{k})\right\}^{2}= 0\), then \(\left\|D^{-1}_{k}B_{k}^{2}D^{-1}_{k}\right\|= 0\).
On the  Figure \ref{fig:localMLE} both the modelling bias and the difference between the widths of the bootstrap and MC confidence bands are close to zero in the regions where the true function \(f(x)\) is constant.
Thus the numerical experiment is consistent with the theoretical results from Section \ref{sect:mainres} and confirm that:
 \begin{itemize}
\item In the case when a (local) parametric model is close to the true distribution the simultaneous bootstrap confidence set is valid. Otherwise the multiplier bootstrap procedure is conservative.
\item The modelling bias widens the simultaneous bootstrap confidence set.
The modelling bias equals to zero for the parametric models that contain the true distribution, and increases up to \(1\) for those parametric models which are farther from the true distribution.
\end{itemize}


\begin{comment}
 \begin{itemize}
 \item[1.]  The simultaneous bootstrap confidence set is widened by the modelling bias.
The closer is a (local) parametric model to the true distribution, the closer is the width of the bootstrap confidence set to the real one (for this particular model).  
 \item[2.] The modelling bias equals to zero for the parametric models which contain the true distribution, and increases up to \(1\) for those parametric models which are farther from the true distribution.
 \end{itemize}
\end{comment}

\begin{figure}[!h]
\caption{ Confidence bands, their widths, and the modelling bias}
\label{fig:localMLE}
%\begin{table}[!h]
\begin{center}
  \begin{tabular}{ c c }
   % \vspace{0.2cm}
\hspace{-1.9cm}   {\Scale[0.85]{\text{bandwidth} \(=\,0.12\)}}
&
\hspace{-1.4cm}   {\Scale[0.85]{\text{bandwidth} \(=\,0.3\)}}\\
%   \multicolumn{2}{c}{Item}\\
\hspace{-1.9cm}  \includegraphics[width=0.522\textwidth]{h=0_12_var=1__1_cut}%{sin025_Lap_n=50_cut1.png}
&
\hspace{-1.4cm}
\includegraphics[width=0.5\textwidth]{h=0_3_var=1__1_cut}%{sin125_Lap_n=50_cut1.png}
  \\
\hspace{-1.9cm}
  \includegraphics[width=0.523\textwidth]{h=0_12_var=1_width_1_cut}%{sin025_Lap_n=50_cut1.png}
&
\hspace{-1.4cm}
\includegraphics[width=0.5\textwidth]{h=0_3_var=1_width_1_cut}%{sin125_Lap_n=50_cut1.png}
\\
\hspace{-1.9cm}
  \includegraphics[width=0.523\textwidth]{bias_h=0_12_cut}
  &
  \hspace{-1.4cm}
   \includegraphics[width=0.5\textwidth]{bias_h=0_3_cut}
  \\
    \multicolumn{2}{c}{
   {\Scale[0.85]{\text{Legend for the top graphs:}}}}\\
    \multicolumn{1}{l}{
%\begin{picture}(0,1)
%\thicklines
%\put(0,2){{\color{black}\line(1,0){15}}}
%\end{picture}
\includegraphics[width=0.08\textwidth]{legend_boot}
%\hspace{0.7cm}
 {{\Scale[0.85]{ \(90\%\) \text{ bootstrap simultaneous confidence band}}}}
  }
 &
 \multicolumn{1}{l}{
~~ \includegraphics[width=0.08\textwidth]{legend_true}
  \,{\(\Scale[0.85]{\text{the true function } f(x)}\)}
  }
 \\
 \multicolumn{1}{l}{
%\begin{picture}(0,1)
%\thicklines
%\put(0,2){{\color{darkgray}\line(1,0){15}}}
%\end{picture}
%\hspace{0.7cm}
\includegraphics[width=0.08\textwidth]{legend_MC}
 {\Scale[0.85]{\(90\%\)\text{ MC simultaneous confidence band}}}}
   &
 \multicolumn{1}{l}{
~~ \includegraphics[width=0.08\textwidth]{legend_localMLE}
  ~{\Scale[0.85]{\text{local constant MLE}}}
  }
  \\
 \multicolumn{2}{l}{
  \includegraphics[width=0.08\textwidth]{legend_smoothed}
  ~{\Scale[0.85]{\text{smoothed target function}}}}\\
  \multicolumn{2}{c}{
   {\Scale[0.85]{\text{Legend for the middle and the bottom graphs:}}}}\\
 \multicolumn{2}{l}{
\includegraphics[width=0.08\textwidth]{legend_boot}
%\hspace{0.7cm}
 {{\Scale[0.85]{\text{width of the } \(90\%\) \text{ bootstrap confidence bands from the upper graphs}}}}
  }\\
  \multicolumn{2}{l}{
\includegraphics[width=0.08\textwidth]{legend_MC}
%\hspace{0.7cm}
 {{\Scale[0.85]{ \text{width of the }\(90\%\)\text{ MC confidence bands from the upper graphs}}}}
  }\\
   \multicolumn{2}{l}{
\includegraphics[width=0.08\textwidth]{legend_bias}
%\hspace{0.7cm}
 {{\Scale[0.85]{ \text{modelling bias from the expression \eqref{eq:numer_smb}} }}}
  }
\\
\multicolumn{2}{l}{\( \)}
\\
\multicolumn{2}{l}{\( \)}
   \end{tabular}
\end{center}
%\end{table}
\end{figure}
\subsection{Effective coverage probability}

In this part of the experiment we check the bootstrap validity by performing many independent simulations. For each of independent \(5000\) \(\{Y_{i}\}\sim \eqref{def:numer_Y}\) samples we took \(10^{4}\) independent bootstrap samples \(\{u_{i}\}\sim \mathcal{N}(1,1)\), and constructed simultaneous bootstrap confidence sets for a range of confidence levels. The second row of  Table \ref{fig:localMLE} contains this range  \((1-\alpha)=0.95, 0.9,\dots, 0.5\). % for which the simultaneous bootstrap confidence sets are constructed.
The third and the fourth lines of Table \ref{fig:localMLE} show the frequencies of the event
$$\max_{1\leq k \leq \numK}\left\{L_{k}(\thetavt_{k})-L_{k}(\thetavs_{k})-\zzb_{k}(\qqqb(\alpha))\right\}\leq 0$$
among \(5000\) data samples, for the bandwidths \(h=0.12, 0.3\), and for the range of \((1-\alpha)\). The results show that the bootstrap procedure is conservative for  both \(h=0.12\) and \(h=0.3\), however, the larger bandwidth yields bigger coverage probabilities.
\begin{table}[!h]
\caption{Effective coverage probabilities for the local constant regression}
\label{tab:cover_eff}
\begin{center}
%\renewcommand{\arraystretch}{1.1}
\scalebox{0.9}{
  \begin{tabular}{| c | c|c|c|c|c |c|c|c|c|c| }  \cline{2-11}
  \multicolumn{1}{c|}{}&\multicolumn{10}{c|}{{{Confidence levels}}}\\\hline
%  \( n \)&\(\mathcal{L}(u_{i})\)&
\(h\)&$\scale[1]{\mathbf{0.95}}$ &\(\scale[1]{\mathbf{0.90}}\) &$\scale[1]{\mathbf{0.85}}$& \(\scale[1]{\mathbf{0.80}}\)& \(\scale[1]{\mathbf{0.75}}\)& \(\scale[1]{\mathbf{0.70}}\)&\(\scale[1]{\mathbf{0.65}}\)&\(\scale[1]{\mathbf{0.60}}\) & \(\scale[1]{\mathbf{0.55}}\)&\(\scale[1]{\mathbf{0.50}}\)\\
\hline\hline
%\multirow{2}[2]*{\(50\)}& \multirow{2}[2]*{\(\mathcal{N}(1,1)\)}&
\(\scale[1]{0.12}\)&
 \(0.971\) & \(0.947\)& \(0.917\) & \(0.888\) &\( 0.863\) &\(0.830\)&\(0.800\)&\( 0.769\)&\(0.738\)&\(0.702\)
  \\ \hline%\cline{3-9}%\hline
%&&
\(\scale[1]{0.3}\)&\(\scale[1]{0.982}\)&\(\scale[1]{0.963}\)&\(\scale[1]{0.942}\)&\(\scale[1]{0.918}\)&\(\scale[1]{0.895}\)&\(\scale[1]{0.868}\)&\(\scale[1]{0.842}\)&
\(\scale[1]{0.815}\)&\(\scale[1]{0.784}\)& \(\scale[1]{0.750}\)\\
\hline
\end{tabular}
}
%\vspace*{-0.3cm}
\end{center}
\end{table}

\subsection{Correction for multiplicity}
Here we compare the \(\Ym\) and the bootstrap corrections for multiplicity, i.e. the values \(\qqq(\alpha)\) and
\(\qqqb(\alpha)\) defined in \eqref{bound:simult} and \eqref{def:mcorrqb}.
The numerical results in Table \ref{tab:corr} are based on  \(10^{4}\) \(\{Y_{i}\}\sim \eqref{def:numer_Y}\) independent samples and \(10^{4}\) independent bootstrap samples \(\{u_{i}\}\sim \mathcal{N}(1,1)\). The second line in Table \ref{tab:corr} contains the range of the nominal confidence levels  \((1-\alpha)=0.95, 0.9,\dots, 0.5\) (similarly to the Table \ref{tab:cover_eff}). The first column contains the values of the bandwidth \(h=0.12, 0.3\), and the second column -- the resampling scheme: Monte Carlo (MC) or bootstrap (B). The Monte Carlo experiment yields the corrected confidence levels \(1-\qqq(\alpha)\), and the bootstrap yields \(1-\qqqb(\alpha)\).
The lines 3--6 show the average values of \(1-\qqq(\alpha)\) and \(1-\qqqb(\alpha)\) over all the experiments. For the smaller bandwidth both the MC and bootstrap corrections are bigger, than the ones for the larger bandwidth.
In the case of the smaller bandwidth the local models have less intersections with each other, and hence, the corrections for multiplicity are closer to the Bonferroni's bound.
\begin{comment}
Another observation from the Table \ref{tab:corr} is that for the bigger bandwidth (and, therefore, for the bigger modelling bias) the difference between bootstrap and MC corrected confidence levels is larger, than in the case of a smaller bandwidth. This is consistent with the one-sided inequality \eqref{ineq:th2qqq} from Theorem \ref{thm:mainres2_largesmb}.
\end{comment}
\begin{table}[!h]
\caption{MC vs Bootstrap confidence levels corrected for multiplicity}
\label{tab:corr}
\begin{center}
%\renewcommand{\arraystretch}{1.1}
\scalebox{0.87}{
  \begin{tabular}{| c | c | c|c|c|c|c |c|c|c|c|c| }  \cline{3-12}
  \multicolumn{2}{c|}{}&\multicolumn{10}{c|}{{{Confidence levels}}}\\\hline
%  \( n \)&\(\mathcal{L}(u_{i})\)&
\(h\)&\(\scale[1]{\text{r.m.}}\)&$\scale[1]{\mathbf{0.95}}$ &\(\scale[1]{\mathbf{0.90}}\) &$\scale[1]{\mathbf{0.85}}$& \(\scale[1]{\mathbf{0.80}}\)& \(\scale[1]{\mathbf{0.75}}\)& \(\scale[1]{\mathbf{0.70}}\)&\(\scale[1]{\mathbf{0.65}}\)&\(\scale[1]{\mathbf{0.60}}\) & \(\scale[1]{\mathbf{0.55}}\)&\(\scale[1]{\mathbf{0.50}}\)\\
\hline\hline
%\multirow{2}[2]*{\(50\)}& \multirow{2}[2]*{\(\mathcal{N}(1,1)\)}&
\multirow{2}[2]*{\(0.12\)}&MC &
 \(0.997\) & \(0.994\)& \(0.989\) & \(0.985\) &\(0.980\) &\(0.975\)&\(0.969\)&\(0.963\)&\(0.956\)&\(0.949\)
   \\ \cline{2-12}
&B &
 \(0.998\) & \(0.995\)& \(0.991\) & \(0.988\) &\(0.984\) &\(0.979\)&\(0.975\)&\(0.969\)&\(0.963\)&\(0.957\)
  \\ \hline\hline%\cline{3-9}%\hline
%&&
\multirow{2}[2]*{\(0.3\)}&MC&\(\scale[1]{0.993}\)&\(\scale[1]{0.983}\)&\(\scale[1]{0.973}\)&\(\scale[1]{0.962}\)&\(\scale[1]{0.949}\)&\(\scale[1]{0.936 }\)&\(\scale[1]{0.922}\)&
\(\scale[1]{0.906}\)&\(\scale[1]{0.891}\)& \(\scale[1]{0.873}\)
\\ \cline{2-12}
&B&\(\scale[1]{0.994}\)&\(\scale[1]{0.986}\)&\(\scale[1]{0.977}\)&\(\scale[1]{0.968}\)&\(\scale[1]{0.958}\)&\(\scale[1]{ 0.947}\)&\(\scale[1]{0.935}\)&
\(\scale[1]{0.922}\)&\(\scale[1]{0.908}\)& \(\scale[1]{0.893}\)\\
\hline
\end{tabular}
}
%\vspace*{-0.3cm}
\end{center}
\end{table}

